Integrating Terrestrial and Non-terrestrial Networks: 3D Opportunities and Challenges

Integrating terrestrial and non-terrestrial networks has the potential of connecting the unconnected and enhancing the user experience for the already-connected, with technological and societal implications of the greatest long-term significance. A convergence of ground, air, and space wireless communications also represents a formidable endeavor for the mobile and satellite communications industries alike, as it entails defining and intelligently orchestrating a new 3D wireless network architecture. In this article, we present the key opportunities and challenges arising from this (r)evolution by presenting some of its disruptive use-cases and key building blocks, reviewing the relevant standardization activities, and pointing to open research problems. By considering two multi-operator paradigms, we also showcase how terrestrial networks could be efficiently re-engineered to cater for aerial services, or opportunistically complemented by non-terrestrial infrastructure to augment their current capabilities.

==> 09_Acknoledgments.tex <==
\section*{Acknowledgments}

==> 0Z_Table_Use-cases.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}
\vspace{1mm}
\caption{Use-cases and scenarios.} 
\label{tab:Use-cases}
\centering
\colorbox{BackgroundGray}{%
\begin{tabular}{ |m{6.5cm}|m{3.5cm}|m{5.0cm}| } 
\toprule
\rowcolor{BackgroundLightBlue}
 \textbf{Critical communications} & \textbf{Availability / Rates / Latency} & \textbf{Benefits of integrated TN-NTN} \\ \midrule
%%%
{Ultra-high definition video up/download in building fires}    & 
{High / High / Low} & 
{Satellite/cellular backhaul to UAV radio access nodes}  \\
\midrule
%%%
{Low-latency remote control of robots in hazardous situations, e.g., wildfire management}    & 
{High / High / Low} & 
{Satellite/cellular backhaul to UAV radio access nodes. Low latency, fast uplink to LEO and aggregation.}  \\
\midrule
%%%
{Replacement coverage in major natural disasters when the ground network becomes dysfunctional}    & 
{High / High / Low} & 
{Satellite/HAPS direct access}  \\
\bottomrule 
%%%
\toprule
\rowcolor{BackgroundLightBlue}
 \textbf{Massive IoT communications} & \textbf{Availability / Rates / Latency} & \textbf{Benefits of integrated TN-NTN} \\ \midrule
%%%
{Remote control of ground, aerial, and maritime vehicles, collecting and sharing real-time data}    & 
{High / Low / Low} & 
{Direct LEO satellite access or via aerial repeaters for massive IoT low-cost devices and delay-tolerant applications}  \\
\midrule
%%%
{Multicast of environmental and mapping information to vehicles}    & 
{High / Low / Medium} & 
{Multicast over LEO satellite to reduce ground segment traffic}  \\
\bottomrule
%%%
\toprule
\rowcolor{BackgroundLightBlue}
 \textbf{\red{Immersive communications?}} & \textbf{Availability / Rates / Latency} & \textbf{Benefits of integrated TN-NTN} \\ \midrule
%%%
{Broadband to moving platforms with control \& user plane separation}    & 
{Medium / High / Low} & 
{Higher reliability for fast-moving platforms. Offloading of control plane and handover traffic from ground segment.}  \\
\bottomrule
%%%
\toprule
\rowcolor{BackgroundLightBlue}
 \textbf{Aerial communications} & \textbf{Availability / Rates / Latency} & \textbf{Benefits of integrated TN-NTN} \\ \midrule
%%%
{City-to-city and last-mile delivery through network-controlled cargo UAVs}    & 
{High / Med / Low} & 
{Hybrid satellite/cellular coverage of 3D aerial corridors}  \\
\midrule
%%%
{Offloading of computationally intensive tasks from UAV swarms (e.g., object recognition and AI-driven autonomous navigation)}    & 
{High / High / Low} & 
{Stable broadband UAV connectivity to the cloud}  \\
\midrule
%%%
{Aircraft in-flight connectivity}    & 
{Med / High / Med} & 
{Broadband coverage of airspace at ~10-15km over both urban areas and oceans}  \\
\bottomrule
\end{tabular}
}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
